Generative deep learning for decision making in gas networks

A decision support system relies on frequent re-solving of similar problem instances. While the general structure remains the same in corresponding applications, the input parameters are updated on a regular basis. We propose a generative neural network design for learning integer decision variables of mixed-integer linear programming (MILP) formulations of these problems. We utilise a deep neural network discriminator and a MILP solver as our oracle to train our generative neural network. In this article, we present the results of our design applied to the transient gas optimisation problem. With the trained network we produce a feasible solution in 2.5s, use it as a warm-start solution, and thereby decrease global optimal solution solve time by 60.5%.

==> sections/actor-critic.tex <==
Good assignments for integer variables of a mixed-integer program (MIP) could also be learned through reinforcement learning. Using the algorithm REINFORCE \cite{thomas2017policy}, a policy could be learned (e.g. using a DNN) , that assigns values to the integer variables. This method could furthermore benefit if we do not only approximate the optimal policy, but also the value function as it is done in actor-critic algorithms (e.g. \cite{pfau2016connecting}). 

Finding good assignments for integer variables in a MIP can be seen as a 1-step Markov Decision Process (MDP). To phrase our problem in reinforcement learning terminology, we describe the  state space,  action  space  and  the  reward  function.

The \textit{state space} is given by (a subset of) the parameters defining the original mixed-integer program combined with the assignments of the binary variables for operation modes. At the beginning, i.e. step 0 of the MDP, we do not have any information about the operation modes. Therefore we do not need to include them as input for our policy approximation.

The \textit{action space} is given by all possible assignments for the binary values that model operation mode choices. So a policy chooses an action for a given state which misses operation modes and therefore completes the state

The \textit{reward function} is given by the objective value of the MIP that is described by the state, e.g. the original MIP for which the operation modes are fixed.



==> sections/solveTimesTable.tex <==
\begin{table}[!ht]
\centering
\begin{small}
\begin{tabular}{lrrrrr}
\toprule
{} &     Mean &  Median &      STD &    Min &       Max \\
\midrule
\neuralnetwork Inference Time (s)               &    0.009 &   0.008 &    0.001 &  0.008 &     0.017 \\
Warmstarted \mip Time (s)                        &  100.830 &   9.380 &  421.084 &  0.130 &  3600.770 \\
\mip Time (s)                                    &  147.893 &  24.380 &  463.279 &  3.600 &  3601.280 \\
\fixedapproxmip + Warmstarted \mip Time (s) &  103.329 &  12.130 &  424.543 &  0.190 &  3726.110 \\
\fixedapproxmip Time (s)                        &    2.499 &   1.380 &   12.714 &  0.060 &   889.380 \\
\bottomrule
\end{tabular}
\end{small}
\caption{Solve time statistics for different solving strategies.}
\label{tab:solve_times}
\end{table}





==> sections/warmStartTable.tex <==
\begin{table}
\centering
\begin{small}
\begin{tabular}{lrr}
\toprule
{}                          & All Instances & MIP Time Limit \\
\midrule
All Instances               &  8640         &  124 \\
Warm Start Successful       &  6040         &  31   \\
Warm Start Not Successful   &  2600         &  93   \\
Warm Start Time Limit       &  16           &  13    \\
\bottomrule
\end{tabular}
\end{small}
\caption{This table show the number of instances that could (could not) be warm-started and that ran into time limit when warm-started (not warm started).}
\label{tab:warm_start}
\end{table}
